An Empirical Evaluation of Sketched SVD and its Application to Leverage Score Ordering

The power of randomized algorithms in numerical methods have led to fast solutions which use the Singular Value Decomposition (SVD) as a core routine. However, given the large data size of modern and the modest runtime of SVD, most practical algorithms would require some form of approximation, such as sketching, when running SVD. While these approximation methods satisfy many theoretical guarantees, we provide the first algorithmic implementations for sketch-and-solve SVD problems on real-world, large-scale datasets. We provide a comprehensive empirical evaluation of these algorithms and provide guidelines on how to ensure accurate deployment to real-world data. As an application of sketched SVD, we present Sketched Leverage Score Ordering, a technique for determining the ordering of data in the training of neural networks. Our technique is based on the distributed computation of leverage scores using random projections. These computed leverage scores provide a flexible and efficient method to determine the optimal ordering of training data without manual intervention or annotations. We present empirical results on an extensive set of experiments across image classification, language sentiment analysis, and multi-modal sentiment analysis. Our method is faster compared to standard randomized projection algorithms and shows improvements in convergence and results.

==> figs.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c : c : c : c}
\Xhline{3\arrayrulewidth}
\multicolumn{5}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
\Xhline{0.5\arrayrulewidth}
\multicolumn{1}{c:}{LR $\rightarrow$ LR} & \multicolumn{1}{c:}{DAN Small $\rightarrow$ LR} & \multicolumn{1}{c:}{DAN Large $\rightarrow$ LR} & \multicolumn{1}{c:}{LSTM Small $\rightarrow$ LR} & \multicolumn{1}{c}{LSTM Large $\rightarrow$ LR} \\ 
\Xhline{0.5\arrayrulewidth}
\includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_0.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_1.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_2.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_3.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_4.png} \\
\includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_0.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_1.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_2.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_3.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_4.png} \\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
\multicolumn{1}{c:}{LR $\rightarrow$ DAN Small} & \multicolumn{1}{c:}{DAN Small $\rightarrow$ DAN Small} & \multicolumn{1}{c:}{DAN Large $\rightarrow$ DAN Small} & \multicolumn{1}{c:}{LSTM Small $\rightarrow$ DAN Small} & \multicolumn{1}{c}{LSTM Large $\rightarrow$ DAN Small} \\ 
\Xhline{0.5\arrayrulewidth}
\includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_5.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_6.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_7.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_8.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_9.png} \\
\includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_5.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_6.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_7.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_8.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_9.png} \\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
\multicolumn{1}{c:}{LR $\rightarrow$ DAN Large} & \multicolumn{1}{c:}{DAN Small $\rightarrow$ DAN Large} & \multicolumn{1}{c:}{DAN Large $\rightarrow$ DAN Large} & \multicolumn{1}{c:}{LSTM Small $\rightarrow$ DAN Large} & \multicolumn{1}{c}{LSTM Large $\rightarrow$ DAN Large} \\ 
\Xhline{0.5\arrayrulewidth}
\includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_10.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_11.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_12.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_13.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_train_14.png} \\
\includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_10.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_11.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_12.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_13.png} & \includegraphics[width=0.22\textwidth]{figs/mosi_late0_valid_14.png} \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Training and Validation MAE curves on CMU-MOSI dataset using a late fusion method, run 0. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001. Notation used to indicate the method is Unimodal Model $\rightarrow$ Multimodal Model.}
\label{mosi_late_graph}
\end{table}

==> tables/levscores.tex <==
\begin{table}[H]
\fontsize{10}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Data size = $n \times$ 50 & \multicolumn{5}{c}{Running Time in Seconds} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
$n =$      & $2^{16}$ & $2^{18}$ & $2^{20}$ & $2^{22}$ & $2^{24}$  \\ 
\Xhline{0.5\arrayrulewidth}
Sketching & 0.9 & 3.3 & 5.4 & 13.5 & 122.5 \\
SVD & 0.7 & 3.3 & 13.9 & 57.2 & 2114.0 \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Running time for Synthetic Data. Sketching's $\epsilon=0.25$}
\label{levscores}
\end{table}

==> tables/mnist0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle	& 91.65 & 96.21 & \textbf{97.78} & 98.53 & 98.90 \\
shuffle     & 91.81 & 96.19 & 97.54 & \textbf{98.66} & 98.90 \\
inc 	& 91.51 & 96.19 & 97.39 & 98.38 & 98.87 \\
dec 	& 91.68 & 95.77 & 97.30 & 98.38 & 98.74 \\
inc, samp w rep	& 91.62 & 96.10 & 97.32 & 98.49 & 98.96 \\
inc, samp wo rep	& \textbf{91.84} & 96.19 & 97.69 & 98.50 & \textbf{99.02} \\
dec, samp w rep	& 91.59 & 95.88 & 97.45 & 98.54 & 98.97 \\
dec, samp wo rep	& 91.59 & \textbf{96.24} & 97.64 & 98.52 & 98.90 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset, run 0. 50 epochs, batchsize 128, SGD optimizer learning rate 0.01.}
\label{mnist0}
\end{table}

==> tables/mnist1.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle			& 92.42 & 98.02 & 97.96 & 98.76 & 98.80 \\
shuffle     		& 92.53 & 98.12 & \textbf{98.19} & 98.83 & 99.10 \\
inc	& 91.19 & 97.59 & 97.02 & 98.67 & 98.87 \\
dec	& 91.43 & 97.26 & 96.67 & 98.65 & 98.73 \\
inc, samp w rep	& 92.24 & 97.74 & 97.53 & 98.80 & 99.10 \\
inc, samp wo rep	& \textbf{92.54} & 98.04 & 97.94 & 98.62 & \textbf{99.20} \\
dec, samp w rep	& 92.12 & 97.86 & 98.07 & 98.66 & 99.06 \\
dec, samp wo rep	& 92.48 & \textbf{98.14} & 97.95 & \textbf{98.96} & 99.16 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset, run 1. 10 epochs, batchsize 200, Adam optimizer learning rate 0.001.}
\label{mnist1}
\end{table}

==> tables/mnist2.tex <==
\begin{table}[t!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle			& 92.77 & 98.40 & 98.72 & 98.86 & 99.33 \\
shuffle     		& 92.68 & \textbf{98.45} & \textbf{98.72} & 99.00 & 99.25 \\
inc	& 91.06 & 98.51 & 98.27 & \textbf{99.07} & 99.18 \\
dec	& 90.69 & 98.51 & 98.23 & 99.06 & 99.30 \\
inc, samp w rep	& 92.65 & 98.18 & 97.98 & 98.72 & 99.25 \\
inc, samp wo rep	& \textbf{92.85} & 98.44 & 98.37 & 98.97 & \textbf{99.34} \\
dec, samp w rep	& 92.45 & 98.05 & 98.14 & 98.78 & 99.23 \\
dec, samp wo rep	& 92.66 & 98.36 & 98.58 & 99.03 & 99.17 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset, run 2. 50 epochs, batchsize 200, Adam optimizer learning rate 0.001.}
\label{mnist2}
\end{table}

==> tables/mnist3.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle			& \textbf{92.86} & 98.25 & 98.52 & 98.98 & 99.18 \\
shuffle     		& 92.75 & \textbf{98.39} & \textbf{98.60} & 99.08 & 99.27 \\
inc	& 91.67 & 98.32 & 97.93 & 98.99 & \textbf{99.35} \\
dec	& 91.54 & 98.17 & 98.23 & 98.96 & 99.31 \\
inc, samp w rep	& 92.78 & 97.97 & 98.26 & 98.99 & 99.23 \\
inc, samp wo rep	& 92.79 & 98.32 & 98.11 & 98.97 & 99.32 \\
dec, samp w rep	& 92.55 & 97.90 & 98.31 & 98.95 & 99.30 \\
dec, samp wo rep	& 92.60 & 98.27 & 98.50 & \textbf{99.13} & 99.18 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset, run 3. 50 epochs, batchsize 128, Adam optimizer learning rate 0.0005.}
\label{mnist3}
\end{table}

==> tables/mnist4.tex <==
\begin{table}[t!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle&92.09&97.33&97.94&98.90&99.14 \\
shuffle&\textbf{92.16}&\textbf{97.37}&\textbf{98.00}&98.80&99.12 \\
inc&91.96&97.30&97.82&98.78&99.08 \\
dec&91.99&97.22&97.77&98.58&99.14 \\
inc, samp w rep&91.97&96.94&97.61&98.64&\textbf{99.28} \\
inc, samp wo rep&92.13&97.36&97.98&98.92&99.23 \\
dec, samp w rep&91.95&97.17&97.62&98.57&99.17 \\
dec, samp wo rep&91.92&97.35&97.91&\textbf{98.96}&99.22 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset, run 4. 100 epochs, batchsize 128, SGD optimizer learning rate 0.01.}
\label{mnist4}
\end{table}

==> tables/mnist5.tex <==
\begin{table}[t!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle&92.79&98.43&98.42&99.02&99.11\\
shuffle&92.66&98.35&\textbf{98.58}&98.87&99.31\\
inc&91.39&\textbf{98.49}&98.26&98.95&99.34\\
dec&91.13&98.41&98.11&\textbf{99.08}&99.28\\
inc, samp w rep&92.71&97.98&98.17&98.65&99.22\\
inc, samp wo rep&\textbf{92.85}&98.31&98.29&98.96&\textbf{99.39}\\
dec, samp w rep&92.42&98.03&98.31&98.82&99.26\\
dec, samp wo rep&92.61&98.40&98.47&98.91&99.32\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset, run 5. 50 epochs, batchsize 256, Adam optimizer learning rate 0.001.}
\label{mnist5}
\end{table}

==> tables/mosi0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR} & \multicolumn{5}{c:}{DAN Small} & \multicolumn{5}{c:}{DAN Large} & \multicolumn{5}{c:}{LSTM Small} & \multicolumn{5}{c}{LSTM Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 67.5&67.1&25.5&\textbf{1.198}&\textbf{0.515}&72.4&72.5&28.1&1.090&0.595&73.3&73.4&29.3&1.033&0.621&74.8&74.8&33.8&0.998&0.643&75.2&75.1&31.8&1.010&0.629 \\
shuffle     & 65.5&65.0&24.1&1.207&0.496&73.6&73.7&27.0&1.087&0.586&75.2&75.3&25.9&1.072&0.612&74.2&74.2&27.8&1.052&0.611&73.2&73.0&30.9&0.996&0.614 \\
inc 	& 63.6&62.7&24.5&1.227&0.499&73.9&74.0&\textbf{28.3}&1.085&0.603&74.1&74.1&28.0&1.060&0.613&74.5&74.4&31.3&1.022&0.629&73.3&72.9&29.3&1.030&0.612 \\
dec 	& \textbf{69.8}&\textbf{69.8}&25.5&1.214&0.516&74.6&74.7&28.6&1.105&0.585&73.3&73.3&27.6&1.070&0.602&73.2&73.0&33.4&0.996&0.627&75.8&75.6&34.1&0.986&0.618 \\
inc, samp w rep	& 63.8&62.7&23.9&1.263&0.501&70.3&70.3&26.5&1.131&0.575&71.1&71.2&28.0&1.096&0.578&72.7&72.7&29.4&1.051&0.598&73.3&73.4&30.2&1.054&0.598 \\
inc, samp wo rep	& 68.2&67.8&27.8&1.199&0.550&73.9&74.0&26.8&\textbf{1.079}&0.603&74.3&74.3&27.6&1.027&0.624&75.2&75.3&32.7&1.041&0.641&74.6&74.6&30.9&1.044&0.631 \\
dec, samp w rep	& 60.8&58.7&24.2&1.280&0.458&71.4&71.5&24.8&1.152&0.535&73.6&73.3&28.1&1.050&0.585&70.7&70.8&27.7&1.074&0.586&73.9&73.9&30.2&1.061&0.590 \\
dec, samp wo rep	& 66.3&65.9&\textbf{25.7}&1.200&0.510&\textbf{74.6}&\textbf{74.7}&27.8&1.088&\textbf{0.607}&73.9&74.0&27.4&1.069&0.602&74.5&74.6&33.1&1.016&0.644&72.6&72.7&31.8&1.047&0.607 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset, run 0. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001.}
\label{mosi0}
\end{table}

==> tables/mosi1.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR} & \multicolumn{5}{c:}{DAN Small} & \multicolumn{5}{c:}{DAN Large} & \multicolumn{5}{c:}{LSTM Small} & \multicolumn{5}{c}{LSTM Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 69.2&69.1&25.7&1.184&0.521&73.9&74.0&27.3&1.098&0.600&73.5&73.4&26.8&1.097&0.582&71.3&71.3&30.9&1.077&0.593&72.4&72.5&29.6&1.053&0.590 \\
shuffle     & 66.5&66.3&25.4&1.187&0.518&74.6&74.6&25.9&1.064&0.603&73.3&73.1&28.0&1.074&0.587&72.7&72.8&30.3&1.046&0.603&74.1&74.0&28.1&1.043&0.573\\
inc 	& 68.7&68.4&27.0&1.183&0.533&71.1&71.2&26.7&1.108&0.594&74.3&74.2&25.8&1.047&0.600&72.7&72.8&32.9&1.017&0.615&71.4&71.3&28.4&1.129&0.608 \\
dec 	& 70.3&70.2&25.7&1.207&0.517&74.1&74.1&25.7&1.090&0.595&70.7&70.7&28.7&1.133&0.581&73.0&73.1&30.0&1.037&0.617&73.3&73.4&27.1&1.014&0.621 \\
inc, samp w rep	& 65.9&65.4&25.9&1.226&0.497&73.3&73.3&28.4&1.069&0.583&73.0&72.9&30.2&1.070&0.577&74.5&74.5&32.8&1.011&0.611&69.8&69.4&26.5&1.190&0.630 \\
inc, samp wo rep	& 69.4&69.4&25.5&1.199&0.524&74.9&74.9&26.4&1.062&0.607&74.3&74.3&28.0&1.075&0.606&74.6&74.5&34.7&0.991&0.615&75.1&75.1&30.6&1.019&0.645\\
dec, samp w rep	& 62.4&61.1&24.8&1.265&0.482&71.7&71.8&27.6&1.086&0.584&75.5&75.5&28.9&1.048&0.601&72.0&72.1&28.6&1.056&0.599&73.6&73.7&24.8&1.121&0.605 \\
dec, samp wo rep	& 70.1&70.1&26.5&1.181&0.532&73.8&73.8&27.0&1.076&0.604&73.0&73.1&28.9&1.079&0.610&75.1&75.1&33.7&0.968&0.637&74.6&74.6&27.4&1.032&0.607 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset, run 1. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.005.}
\label{mosi1}
\end{table}

==> tables/mosi_late0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR $\rightarrow$ LR} & \multicolumn{5}{c:}{DAN Small $\rightarrow$ LR} & \multicolumn{5}{c:}{DAN Large $\rightarrow$ LR} & \multicolumn{5}{c:}{LSTM Small $\rightarrow$ LR} & \multicolumn{5}{c}{LSTM Large $\rightarrow$ LR} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 67.9&67.6&25.5&1.200&0.517&72.2&72.2&27.7&1.092&0.589&72.6&72.7&29.6&1.066&0.593&73.3&73.3&31.3&1.033&0.607&70.8&70.9&30.5&1.052&0.591 \\
shuffle     & 65.3&64.5&23.9&1.214&0.502&72.3&72.4&27.8&1.102&0.575&72.0&72.1&28.4&1.086&0.587&74.1&74.1&33.2&1.027&0.610&72.0&72.0&28.1&1.037&0.606 \\
inc 	& 66.9&66.3&24.8&1.215&0.506&72.3&72.4&28.1&1.109&0.566&73.5&73.5&28.3&1.057&0.606&71.6&71.6&31.2&1.057&0.582&72.6&72.7&32.9&1.040&0.600 \\
dec 	& 69.8&69.8&24.6&1.209&0.504&72.2&72.2&27.1&1.128&0.553&74.1&74.1&29.3&1.062&0.599&74.1&74.0&34.0&1.021&0.608&73.6&73.7&30.9&1.041&0.607 \\
inc, samp w rep	& 64.0&63.6&22.2&1.263&0.434&72.6&72.7&29.0&1.125&0.560&70.6&70.6&25.4&1.138&0.547&71.4&71.5&28.9&1.095&0.573&71.0&71.1&25.2&1.150&0.540 \\
inc, samp wo rep	& 70.4&70.3&25.4&1.194&0.518&55.5&53.9&19.2&1.434&0.227&55.1&51.0&15.6&1.425&0.147&52.6&50.1&15.0&1.420&0.135&56.1&52.3&20.4&1.391&0.391 \\
dec, samp w rep	& 69.4&69.3&25.1&1.199&0.510&71.3&71.3&27.3&1.127&0.56&73.9&74.0&29.6&1.072&0.579&71.7&71.8&27.7&1.104&0.560&72.9&73.0&31.8&1.045&0.598 \\
dec, samp wo rep	& 67.2&66.8&26.4&1.198&0.533&71.9&71.9&28.1&1.108&0.576&74.8&74.8&28.3&1.048&0.612&74.3&74.4&28.9&1.068&0.590&73.0&73.1&29.2&1.032&0.611 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
Method       & \multicolumn{5}{c:}{LR $\rightarrow$ DAN Small} & \multicolumn{5}{c:}{DAN Small $\rightarrow$ DAN Small} & \multicolumn{5}{c:}{DAN Large $\rightarrow$ DAN Small} & \multicolumn{5}{c:}{LSTM Small $\rightarrow$ DAN Small} & \multicolumn{5}{c}{LSTM Large $\rightarrow$ DAN Small} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 73.9&73.9&27.3&1.089&0.599&72.6&72.7&27.4&1.065&0.601&74.3&74.4&27.4&1.05&0.597&72.4&72.5&29.7&1.05&0.595&73.2&73.2&29.6&1.032&0.616 \\
shuffle     & 74.3&74.4&27.3&1.076&0.600&72.4&72.5&28.9&1.075&0.593&72.4&72.5&27.7&1.065&0.597&71.0&71.1&29.2&1.065&0.596&74.2&74.2&30.8&1.010&0.619 \\
inc 	& 74.2&74.3&28.6&1.077&0.606&73.6&73.7&28.1&1.074&0.596&73.0&73.1&29.6&1.072&0.592&73.0&73.0&33.4&1.021&0.603&73.3&73.3&31.2&1.016&0.610 \\
dec 	& 74.9&75.0&27.4&1.096&0.573&73.3&73.4&27.3&1.075&0.581&74.5&74.6&27.4&1.055&0.596&72.7&72.8&32.1&1.041&0.593&73.6&73.5&32.4&1.030&0.605 \\
inc, samp w rep	& 70.7&70.7&24.9&1.155&0.565&73.3&73.3&24.8&1.094&0.555&73.0&73.1&28.9&1.048&0.601&72.6&72.7&28.6&1.078&0.594&70.7&70.8&29.9&1.083&0.577 \\
inc, samp wo rep	& 73.6&73.7&27.8&1.081&0.601&57.6&56.2&20.0&1.400&0.289&56.1&54.8&18.2&1.365&0.293&57.7&57.4&19.5&1.364&0.282&53.6&52.0&20.3&1.442&0.182 \\
dec, samp w rep	& 73.2&73.2&27.8&1.102&0.563&73.0&73.1&27.3&1.089&0.586&72.0&72.1&28.3&1.088&0.581&70.0&70.0&29.9&1.073&0.595&72.9&72.9&30.3&1.042&0.607 \\
dec, samp wo rep	& 72.7&72.8&25.9&1.114&0.573&71.3&71.4&27.0&1.077&0.588&73.3&73.3&28.1&1.065&0.598&74.1&74.1&30.3&1.035&0.616&74.8&74.8&32.9&1.000&0.621 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
Method       & \multicolumn{5}{c:}{LR $\rightarrow$ DAN Large} & \multicolumn{5}{c:}{DAN Small $\rightarrow$ DAN Large} & \multicolumn{5}{c:}{DAN Large $\rightarrow$ DAN Large} & \multicolumn{5}{c:}{LSTM Small $\rightarrow$ DAN Large} & \multicolumn{5}{c}{LSTM Large $\rightarrow$ DAN Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 74.5&74.5&28.1&1.032&0.618&72.4&72.5&28.6&1.059&0.602&74.1&74.1&27.8&1.062&0.598&73.0&73.0&29.2&1.057&0.599&74.5&74.3&28.9&1.032&0.605 \\
shuffle     & 74.3&74.3&26.7&1.060&0.611&73.3&73.4&27.4&1.080&0.596&74.6&74.7&28.3&1.045&0.607&75.1&75.0&31.8&1.004&0.635&74.1&74.1&29.6&1.025&0.624 \\
inc 	& 73.9&73.9&27.1&1.089&0.600&74.6&74.6&28.0&1.054&0.615&73.8&73.8&28.6&1.064&0.602&73.2&73.1&30.3&1.035&0.610&74.8&74.5&28.0&1.035&0.614 \\
dec 	& 74.6&74.6&30.3&1.030&0.625&73.0&73.1&26.8&1.079&0.579&74.6&74.7&27.8&1.039&0.601&71.9&71.7&30.3&1.082&0.552&74.2&74.2&26.4&1.031&0.617 \\
inc, samp w rep	& 73.8&73.8&27.3&1.090&0.607&72.7&72.7&25.9&1.108&0.581&72.3&72.3&29.9&1.113&0.569&71.9&71.9&24.9&1.101&0.591&72.6&72.6&27.3&1.069&0.596 \\
inc, samp wo rep	& 75.7&75.7&28.3&1.054&0.614&59.5&59.1&19.5&1.348&0.298&58.3&57.4&18.9&1.402&0.254&56.3&55.1&21.4&1.433&0.260&57.9&57.1&18.2&1.353&0.323 \\
dec, samp w rep	& 72.4&72.5&24.9&1.099&0.577&67.5&67.5&26.5&1.167&0.521&73.2&73.2&26.7&1.099&0.579&72.6&72.6&27.4&1.063&0.600&74.9&74.9&26.8&1.060&0.600 \\
dec, samp wo rep	& 75.5&75.5&28.3&1.026&0.624&71.6&71.6&28.6&1.076&0.581&73.2&73.2&27.3&1.059&0.604&72.4&72.5&29.0&1.04&0.610&74.9&74.9&30.2&1.026&0.620 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset using a late fusion method, run 0. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001. Notation used to indicate the method is Unimodal Model $\rightarrow$ Multimodal Model.}
\label{mosi_late0}
\end{table}

==> tables/mosi_late1.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR $\rightarrow$ LR} & \multicolumn{5}{c:}{DAN Small $\rightarrow$ LR} & \multicolumn{5}{c:}{DAN Large $\rightarrow$ LR} & \multicolumn{5}{c:}{LSTM Small $\rightarrow$ LR} & \multicolumn{5}{c}{LSTM Large $\rightarrow$ LR} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 70.3&70.1&\textbf{28.1}&1.182&0.544&73.2&73.2&28.1&1.088&0.584&72.9&73.0&29.7&1.056&0.596&72.2&72.1&29.4&1.040&0.586&74.5&74.4&32.8&1.001&0.618 \\
shuffle     & 68.8&68.7&25.2&1.193&0.527&71.9&71.9&26.7&1.096&0.575&74.2&74.2&28.4&1.044&0.598&72.2&72.2&33.1&1.046&0.584&73.2&73.2&27.4&1.060&0.590 \\
inc 	& 68.4&68.1&25.1&1.193&0.515&73.2&73.3&27.7&1.081&0.586&73.9&74.0&28.0&1.087&0.589&72.9&73.0&34.1&1.040&0.595&72.3&72.4&29.7&1.099&0.564 \\
dec 	& \textbf{70.8}&\textbf{70.9}&24.2&1.194&0.506&73.8&73.8&26.5&1.114&0.57&74.3&74.4&27.3&1.079&0.584&73.6&73.4&29.7&1.051&0.590&74.9&74.9&32.9&0.997&0.619 \\
inc, samp w rep	& 68.4&68.3&26.5&1.178&0.508&73.8&73.8&27.1&1.104&0.591&74.2&74.3&28.4&1.102&0.568&68.8&68.9&25.9&1.121&0.528&70.6&70.6&26.2&1.100&0.568 \\
inc, samp wo rep	& 69.0&68.6&27.8&1.200&\textbf{0.547}&54.1&49.8&18.7&1.434&0.288&50.0&42.7&16.0&1.443&0.203&54.5&53.2&18.9&1.418&0.222&50.3&48.0&16.8&1.455&0.124 \\
dec, samp w rep	& 66.0&65.9&22.4&1.261&0.428&71.0&71.0&27.0&1.129&0.561&70.1&70.2&27.1&1.117&0.559&70.1&70.2&28.1&1.124&0.550&71.6&71.6&29.2&1.060&0.582 \\
dec, samp wo rep	& 70.8&70.8&25.4&\textbf{1.168}&0.545&73.6&73.7&28.3&1.067&0.596&72.7&72.8&29.4&1.096&0.591&71.0&71.1&29.7&1.061&0.577&71.9&71.9&32.7&1.020&0.602  \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
Method       & \multicolumn{5}{c:}{LR $\rightarrow$ DAN Small} & \multicolumn{5}{c:}{DAN Small $\rightarrow$ DAN Small} & \multicolumn{5}{c:}{DAN Large $\rightarrow$ DAN Small} & \multicolumn{5}{c:}{LSTM Small $\rightarrow$ DAN Small} & \multicolumn{5}{c}{LSTM Large $\rightarrow$ DAN Small} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 74.5&74.6&25.2&1.072&0.600&74.1&74.1&28.6&1.043&0.604&74.2&74.2&27.7&1.064&0.602&72.0&72.0&29.7&1.049&0.583&72.6&72.6&33.1&1.034&0.602 \\
shuffle     & 73.8&73.8&25.7&1.086&0.587&72.7&72.7&29.0&1.033&0.607&71.0&71.0&27.6&1.077&0.572&72.6&72.6&29.0&1.106&0.561&74.8&74.8&30.3&1.017&0.617 \\
inc 	& 73.9&73.9&26.1&1.086&0.595&73.6&73.7&27.8&1.059&0.600&73.8&73.8&29.2&1.060&0.603&72.3&72.3&31.2&1.084&0.559&72.0&72.0&32.7&1.032&0.596 \\
dec 	& 74.1&74.1&26.4&1.112&0.575&72.4&72.5&28.9&1.083&0.576&71.0&71.1&26.8&1.082&0.556&73.5&73.5&29.7&1.046&0.589&72.3&72.2&31.1&1.027&0.594 \\
inc, samp w rep	& 72.3&72.4&25.2&1.182&0.518&73.3&73.4&27.0&1.087&0.577&70.3&70.3&27.1&1.105&0.569&74.3&74.4&30.9&1.059&0.583&68.7&68.6&27.8&1.135&0.514 \\
inc, samp wo rep	& 74.3&74.4&28.0&1.058&0.603&55.5&53.7&20.1&1.414&0.260&55.8&53.0&19.1&1.391&0.280&58.2&56.8&18.8&1.376&0.266&57.1&56.5&19.8&1.423&0.212 \\
dec, samp w rep	& 72.4&72.5&27.0&1.112&0.570&73.2&73.3&28.4&1.074&0.592&71.3&71.4&27.3&1.103&0.565&69.8&69.9&26.1&1.166&0.500&73.3&73.4&27.3&1.055&0.593 \\
dec, samp wo rep	& 72.2&72.2&26.4&1.101&0.593&71.9&71.9&29.9&1.076&0.588&73.6&73.7&27.6&1.050&0.605&71.6&71.6&34.1&1.046&0.589&74.3&74.4&31.2&1.030&0.616 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
Method       & \multicolumn{5}{c:}{LR $\rightarrow$ DAN Large} & \multicolumn{5}{c:}{DAN Small $\rightarrow$ DAN Large} & \multicolumn{5}{c:}{DAN Large $\rightarrow$ DAN Large} & \multicolumn{5}{c:}{LSTM Small $\rightarrow$ DAN Large} & \multicolumn{5}{c}{LSTM Large $\rightarrow$ DAN Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle	& 74.2&74.0&26.7&1.046&0.606&73.3&73.4&27.8&1.042&0.602&71.1&71.2&28.6&1.102&0.574&74.5&74.5&27.3&1.092&0.593&74.5&74.4&28.7&1.024&0.611 \\
shuffle     &74.2&74.2&26.8&1.079&0.597&73.2&73.2&27.3&1.098&0.586&74.8&74.8&25.2&1.100&0.615&74.1&74.0&25.9&1.085&0.611&75.4&75.4&27.3&1.055&0.610 \\
inc 	&72.2&72.2&26.4&1.121&0.606&73.2&73.2&28.9&1.084&0.606&72.3&72.4&27.1&1.114&0.567&74.9&74.9&28.0&1.045&0.601&72.9&72.9&28.9&1.061&0.602 \\
dec 	& 71.4&71.4&28.1&1.107&0.592&74.6&74.6&25.7&1.060&0.581&75.2&74.9&26.8&1.039&0.59&71.3&71.4&30.0&1.119&0.557&72.6&72.6&28.3&1.051&0.592 \\
inc, samp w rep	&70.4&70.5&25.4&1.164&0.567&73.0&73.1&29.2&1.107&0.589&73.0&73.0&26.8&1.073&0.596&71.3&71.3&26.7&1.111&0.560&71.1&71.2&26.4&1.096&0.570 \\
inc, samp wo rep	&74.1&74.1&27.4&1.100&0.598&60.3&59.7&22.0&1.348&0.366&56.7&56.1&17.6&1.385&0.264&57.9&55.7&17.6&1.404&0.302&55.5&54.7&18.7&1.400&0.210 \\
dec, samp w rep	&70.8&70.8&25.2&1.115&0.546&71.0&71.0&27.8&1.150&0.569&71.7&71.8&29.4&1.067&0.587&71.7&71.6&27.8&1.103&0.582&71.7&71.8&26.7&1.141&0.558 \\
dec, samp wo rep	&  73.9&73.9&28.7&1.071&0.606&72.2&72.2&29.2&1.064&0.579&72.4&72.5&27.4&1.087&0.599&72.4&72.4&29.6&1.069&0.581&72.4&72.5&28.1&1.043&0.609 \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset using a late fusion method, run 1. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.005. Notation used to indicate the method is Unimodal Model $\rightarrow$ Multimodal Model.}
\label{mosi_late1}
\end{table}

==> tables/sst0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{SST} 5 Class Sentiment Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & DAN Small & DAN Large & LSTM Small & LSTM Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle/shuffle			& 42.99 & 41.95 & 42.08 & 41.18 & 42.13 \\
%shuffle     		& 43.48 & 45.11 & 43.48 & 42.13 & 41.77 \\
inc	& 43.94 & 44.16 & 42.13 & 41.00 & 40.72 \\
dec	& 44.03 & \textbf{45.70} & 40.36 & 40.81 & 42.13 \\
inc, samp w rep	& 43.58 & 40.95 & 40.72 & 38.19 & 42.45 \\
inc, samp wo rep	& \textbf{44.07} & 43.62 & \textbf{43.71} & 40.86 & 41.77 \\
dec, samp w rep	& 43.39 & 41.13 & 41.99 & 41.45 & 40.32 \\
dec, samp wo rep	& 43.71 & 43.94 & 42.44 & \textbf{42.85} & \textbf{43.85} \\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on SST dataset, run 0. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001.}
\label{sst0}
\end{table}

==> tables/sst1.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{SST} 5 Class Sentiment Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & DAN Small & DAN Large & LSTM Small & LSTM Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle &42.53&44.39&43.53&41.09&40.54\\
shuffle &43.76&45.16&42.99&41.90&42.40\\
inc&44.16&\textbf{44.84}&43.44&41.49&42.22\\
dec&43.62&43.98&42.35&41.36&\textbf{43.26}\\
inc, samp w rep&43.26&42.80&40.86&39.73&39.50\\
inc, samp wo rep&\textbf{44.25}&44.57&44.03&41.95&41.22\\
dec, samp w rep&43.35&42.99&41.99&41.22&40.09\\
dec, samp wo rep&43.58&44.21&\textbf{44.30}&\textbf{42.71}&42.85\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on SST dataset, run 1. Epochs determined by validation set, batchsize 256, Adam optimizer, learning rate 0.001.}
\label{sst1}
\end{table}

==> tables/sst2.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{SST} 5 Class Sentiment Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & DAN Small & DAN Large & LSTM Small & LSTM Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle&42.85&45.02&43.58&40.68&42.90\\
shuffle&43.30&45.16&43.53&40.59&43.44\\
inc&\textbf{44.25}&44.84&43.89&39.64&\textbf{44.21}\\
dec&44.12&44.30&43.98&40.50&43.58\\
inc, samp w rep&43.26&43.12&41.40&39.73&39.14\\
inc, samp wo rep&43.85&\textbf{45.61}&43.12&\textbf{42.62}&40.59\\
dec, samp w rep&42.67&42.99&40.72&38.82&41.04\\
dec, samp wo rep&43.71&45.02&\textbf{45.02}&42.31&43.35\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on SST dataset, run 2. Epochs determined by validation set, batchsize 256, Adam optimizer, learning rate 0.0005.}
\label{sst1}
\end{table}

==> tables2/late0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c : c c : c c : c c : c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{10}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{2}{c:}{LR $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{DAN Small $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{DAN Large $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{LSTM Small $\rightarrow$ DAN Large} & \multicolumn{2}{c}{LSTM Large $\rightarrow$ DAN Large} \\ 
Metric & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE \\
\Xhline{0.5\arrayrulewidth}
no shuffle&\textbf{68.1}&1.207&74.6&1.078&72.7&1.066&71.9&1.063&73.0&1.041\\
shuffle&67.3&\textbf{1.180}&73.2&1.072&74.1&1.056&69.5&1.103&73.8&1.027\\
%65.9&64.9&23.0&1.224&0.509&73.6&73.7&26.2&1.111&0.579&73.0&73.1&27.8&1.077&0.573&71.3&71.3&33.1&1.052&0.584&71.7&71.7&29.7&1.036&0.591\\
dec&\textbf{68.1}&1.212&71.3&1.124&71.1&1.086&71.6&1.072&74.1&1.027\\
dec, samp w rep& 67.5&1.194&72.9&1.080&71.6&1.078&72.9&1.021&74.6&1.013\\
dec, samp wo rep& 67.3&1.196&73.5&1.068&73.2&1.049&71.9&1.058&75.4&0.996\\
%66.8&66.4&24.5&1.206&0.501&73.8&73.8&27.6&1.064&0.601&72.6&72.6&30.8&1.053&0.588&73.8&73.8&28.9&1.032&0.61&74.1&74.0&30.9&1.023&0.605\\
%68.7&68.1&22.7&1.201&0.515&72.9&72.9&28.6&1.083&0.587&73.0&73.1&27.6&1.081&0.581&72.9&73.0&31.5&1.051&0.586&71.9&71.9&30.5&1.054&0.577\\
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
Method       & \multicolumn{2}{c:}{LR $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{DAN Small $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{DAN Large $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{LSTM Small $\rightarrow$ DAN Large} & \multicolumn{2}{c}{LSTM Large $\rightarrow$ DAN Large} \\ 
Metric & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE \\
\Xhline{0.5\arrayrulewidth}
no shuffle&74.1&1.062&73.2&1.051&74.5&1.019&70.8&1.063&73.7&1.024\\
shuffle&74.8&1.072&74.3&1.047&75.5&1.024&72.7&1.035&72.7&1.042\\
%74.3&74.4&28.0&1.087&0.598&72.7&72.8&29.0&1.054&0.589&74.3&74.4&30.8&1.023&0.611&71.4&71.4&31.1&1.036&0.578&70.8&70.9&28.0&1.055&0.596&
dec&74.2&1.084&74.1&1.073&72.6&1.043&72.2&1.042&71.6&1.030\\
dec, samp w rep& 74.2&1.080&73.9&1.045&74.3&1.014&72.2&1.061&73.0&1.035\\
dec, samp wo rep& 75.7&1.064&71.6&1.058&72.9&1.054&72.7&1.052&74.3&1.003\\
%75.2&75.2&28.3&1.038&0.606&72.9&73.0&32.1&1.031&0.614&75.9&75.9&29.7&1.013&0.619&72.7&72.8&32.2&1.034&0.584&72.4&72.5&30.5&1.03&0.599&
%74.1&74.1&27.1&1.075&0.606&72.0&72.1&28.3&1.103&0.574&70.7&70.8&31.1&1.088&0.554&71.9&71.9&29.0&1.058&0.589&72.0&72.0&30.6&1.041&0.597&
\Xhline{3\arrayrulewidth}
\\
\Xhline{3\arrayrulewidth}
Method       & \multicolumn{2}{c:}{LR $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{DAN Small $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{DAN Large $\rightarrow$ DAN Large} & \multicolumn{2}{c:}{LSTM Small $\rightarrow$ DAN Large} & \multicolumn{2}{c}{LSTM Large $\rightarrow$ DAN Large} \\ 
Metric & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE & A$^{2}$ & MAE \\
\Xhline{0.5\arrayrulewidth}
no shuffle&73.5&1.056&70.8&1.090&73.2&1.05&73.0&1.035&73.9&1.034\\
shuffle&74.2&1.045&73.8&1.053&73.3&1.054&72.2&1.056&75.1&0.986\\
%73.5&73.5&29.2&1.052&0.614&74.5&74.6&29.0&1.067&0.599&69.7&69.7&31.1&1.074&0.569&74.1&74.1&28.4&1.044&0.578&72.2&72.2&28.6&1.04&0.601&
dec&74.8&1.051&74.1&1.067&71.6&1.100&73.8&1.049&72.7&1.041\\
dec, samp w rep& 72.6&1.072&73.2&1.060&73.3&1.055&71.9&1.069&73.2&1.035\\
dec, samp wo rep& 76.2&1.014&72.9&1.065&73.8&1.057&73.0&1.045&74.6&0.990\\
%73.9&74.0&29.9&1.051&0.611&73.6&73.6&30.8&1.034&0.606&73.9&74.0&30.2&1.055&0.597&72.6&72.6&29.6&1.032&0.599&73.5&73.4&29.4&1.014&0.623&
%75.4&75.3&25.9&1.045&0.62&74.6&74.7&29.0&1.058&0.588&74.5&74.5&29.3&1.046&0.595&73.0&73.0&28.6&1.067&0.582&71.7&71.8&29.7&1.04&0.592&
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset using a late fusion method. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001. Notation used to indicate the method is Unimodal Model $\rightarrow$ Multimodal Model.}
\label{mosi_late0}
\end{table}

==> tables2/mnist1.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle &92.76&98.32&\textbf{98.60}&98.79&99.16\\
shuffle &\textbf{92.81}&98.24&98.39&99.04&\textbf{99.36}\\
%inc &92.09&98.08&98.31&99.01&99.10\\
dec &90.82&\textbf{98.33}&98.28&98.67&98.97\\
dec, samp w rep &92.60&98.25&98.40&99.07&99.31\\
dec, samp wo rep &92.76&98.29&98.54&\textbf{99.12}&99.27\\
%inc, samp w rep &92.79&\textbf{98.36}&98.42&\textbf{99.14}&99.32\\
%inc, samp wo rep &\textbf{92.81}&98.28&98.48&98.95&\textbf{99.40}\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset. 50 epochs, batchsize 256, Adam optimizer learning rate 0.0005.}
\label{mnist1}
\end{table}

==> tables2/mnist2.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{MNIST} 10 Class Image Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & NN Small & NN Large & CNN Small & CNN Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle &91.66&96.19&97.70&\textbf{98.64}&98.86\\
shuffle &\textbf{91.81}&\textbf{96.23}&\textbf{97.85}&98.51&98.95\\
%inc &\textbf{91.86}&96.13&97.66&\textbf{98.71}&99.04\\
dec &91.64&96.14&97.39&98.60&99.00\\
dec, samp w rep &91.58&96.18&97.64&98.52&\textbf{99.06}\\
dec, samp wo rep &91.56&96.13&97.82&\textbf{98.64}&98.97\\
%inc, samp w rep &91.70&96.20&97.61&98.62&\textbf{99.13}\\
%inc, samp wo rep &91.64&\textbf{96.27}&\textbf{97.87}&98.62&98.98\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on MNIST dataset. 100 epochs, batchsize 256, Adam optimizer learning rate 0.001.}
\label{mnist2}
\end{table}

==> tables2/mosi0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR} & \multicolumn{5}{c:}{DAN Small} & \multicolumn{5}{c:}{DAN Large} & \multicolumn{5}{c:}{LSTM Small} & \multicolumn{5}{c}{LSTM Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle &62.4&61.6&17.3&1.336&0.378&71.1&71.2&26.8&1.128&0.570&73.6&73.7&28.6&1.060&0.610&74.1&74.1&30.2&1.061&0.604&74.1&74.1&32.4&1.042&0.600\\
shuffle &61.1&59.3&17.6&1.327&0.454&71.7&71.8&26.4&1.130&0.553&73.8&73.8&26.4&1.083&0.589&73.9&74.0&31.3&1.035&0.616&72.4&72.5&31.5&1.050&0.605\\
%inc &61.2&60.0&16.5&1.356&0.387&70.7&70.7&25.7&1.138&0.560&72.6&72.7&28.6&1.084&0.601&73.5&73.5&30.6&1.025&0.625&70.6&70.6&29.3&1.077&0.593\\
dec &64.6&63.9&20.0&1.289&0.440&72.9&73.0&26.8&1.111&0.578&72.2&72.2&28.9&1.040&0.620&73.5&73.5&31.9&1.029&0.634&71.4&71.5&32.7&1.043&0.614\\
dec samp w rep &65.2&64.3&17.3&1.317&0.449&71.1&71.2&25.7&1.132&0.55&73.3&73.3&28.3&1.076&0.600&75.5&75.6&33.1&1.028&0.643&72.0&72.1&30.0&1.041&0.602\\
dec samp wo rep &62.1&60.0&19.4&1.303&0.464&72.6&72.7&24.1&1.116&0.564&73.6&73.6&28.9&1.068&0.592&73.9&74.0&32.4&1.040&0.636&73.9&74.0&33.1&1.032&0.634\\
%inc samp w rep &56.3&51.6&20.0&1.352&0.426&71.9&71.9&27.3&1.127&0.547&73.6&73.7&27.7&1.093&0.589&73.8&73.8&29.0&1.039&0.618&74.1&73.6&31.5&0.990&0.629\\
%inc samp wo rep &56.9&52.9&15.5&1.369&0.431&70.0&70.0&24.2&1.152&0.534&75.2&75.2&26.2&1.074&0.607&75.2&75.3&29.4&1.014&0.629&74.1&74.0&33.8&1.033&0.615\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001.}
\label{mosi0}
\end{table}

==> tables2/mosi1.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR} & \multicolumn{5}{c:}{DAN Small} & \multicolumn{5}{c:}{DAN Large} & \multicolumn{5}{c:}{LSTM Small} & \multicolumn{5}{c}{LSTM Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle &63.6&62.9&20.8&1.282&0.449&72.9&73.0&\textbf{28.6}&1.085&\textbf{0.597}&73.8&73.8&28.4&1.067&0.612&74.5&74.4&30.0&1.017&0.619&\textbf{75.1}&\textbf{75.1}&30.3&1.048&0.635\\
shuffle &64.6&63.9&22.9&\textbf{1.244}&0.481&\textbf{75.5}&\textbf{75.5}&27.1&\textbf{1.083}&0.580&73.3&73.3&27.1&1.043&0.607&73.5&73.5&31.9&1.038&0.624&71.9&71.9&31.5&1.038&0.611\\
%&65.5&64.6&18.2&1.298&0.461&73.0&73.1&28.1&1.098&0.591&72.6&72.6&29.9&1.059&0.601&70.4&70.4&28.0&1.081&0.604&73.3&73.4&29.9&1.024&0.618\\
dec&\textbf{67.6}&\textbf{67.3}&\textbf{24.1}&1.250&0.461&74.1&74.1&28.0&1.088&0.589&\textbf{74.9}&\textbf{75.0}&\textbf{28.7}&\textbf{1.037}&\textbf{0.618}&73.9&73.7&29.9&1.013&0.627&74.1&74.1&31.6&1.021&\textbf{0.636}\\
dec samp w rep &63.8&62.7&22.3&1.268&0.478&71.7&71.8&26.1&1.105&0.575&73.0&73.0&\textbf{28.7}&1.065&0.604&\textbf{75.7}&\textbf{75.7}&\textbf{33.2}&\textbf{1.005}&\textbf{0.654}&74.5&74.4&31.6&\textbf{1.008}&0.613\\
dec samp wo rep &64.0&62.8&23.8&\textbf{1.244}&\textbf{0.485}&73.9&74.0&24.9&1.093&0.587&74.5&74.5&27.0&1.048&0.613&73.0&73.1&32.1&1.062&0.615&73.0&73.1&\textbf{31.9}&1.032&0.626\\
%&63.4&62.3&22.3&1.258&0.459&72.4&72.5&28.1&1.100&0.573&72.4&72.4&28.1&1.044&0.602&75.1&75.1&32.8&1.026&0.623&74.8&74.8&32.9&1.001&0.631\\
%&64.0&62.8&18.1&1.301&0.462&72.6&72.6&25.8&1.115&0.579&75.8&75.8&27.6&1.063&0.614&75.7&75.7&31.3&1.018&0.634&74.3&74.4&32.8&1.047&0.613\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset. Epochs determined by validation set, batchsize 256, Adam optimizer, learning rate 0.001.}
\label{mosi1}
\end{table}

==> tables2/mosi2.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{1.0pt}
\begin{tabular}{l : c c c c c : c c c c c : c c c c c : c c c c c : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{25}{c}{\textbf{CMU-MOSI} Sentiment Analysis} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & \multicolumn{5}{c:}{LR} & \multicolumn{5}{c:}{DAN Small} & \multicolumn{5}{c:}{DAN Large} & \multicolumn{5}{c:}{LSTM Small} & \multicolumn{5}{c}{LSTM Large} \\ 
Metric & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ & A$^{2}$ & F1 & A$^{7}$ & MAE & $r$ \\
\Xhline{0.5\arrayrulewidth}
no shuffle &66.0&65.5&24.9&1.226&0.492&\textbf{74.9}&\textbf{75.0}&28.3&1.069&0.605&\textbf{73.8}&\textbf{73.8}&30.3&1.056&0.604&72.6&72.7&29.7&1.042&0.608&75.1&74.9&29.9&1.039&0.619\\
shuffle &65.7&65.2&24.9&1.206&0.501&74.1&74.1&27.6&1.082&0.600&74.1&74.0&28.4&\textbf{1.032}&\textbf{0.616}&73.6&73.7&30.6&1.046&0.609&\textbf{75.4}&\textbf{75.0}&31.2&\textbf{0.988}&\textbf{0.629}\\
%&65.9&65.0&23.6&1.227&0.501&74.5&74.5&27.4&1.076&0.605&74.6&74.6&28.1&1.035&0.611&73.8&73.8&30.5&1.028&0.632&72.2&72.2&28.0&1.087&0.606\\
dec&\textbf{69.7}&\textbf{69.6}&\textbf{25.8}&1.214&0.499&\textbf{74.9}&\textbf{75.0}&27.7&1.080&0.598&74.2&74.3&29.3&1.064&0.600&71.9&71.9&28.7&1.042&0.600&73.5&73.5&31.8&1.011&0.615\\
dec, samp w rep &65.5&64.8&23.2&1.216&0.507&73.9&74.0&27.7&1.081&0.603&72.7&72.8&29.9&1.048&0.610&73.3&73.4&\textbf{31.5}&\textbf{1.016}&0.631&74.1&74.0&\textbf{32.7}&1.005&0.614\\
dec, samp wo rep &66.6&66.1&24.5&\textbf{1.202}&\textbf{0.512}&74.2&74.3&\textbf{28.6}&\textbf{1.064}&\textbf{0.612}&73.6&73.7&\textbf{31.2}&1.047&\textbf{0.616}&\textbf{73.8}&\textbf{73.8}&30.0&1.025&\textbf{0.634}&72.3&72.4&31.6&1.047&0.609\\
%&66.6&66.4&24.2&1.203&0.484&73.6&73.7&30.0&1.089&0.587&73.0&73.1&28.0&1.064&0.599&76.1&76.2&32.2&1.002&0.640&75.5&75.5&31.8&0.996&0.637\\
%&65.2&64.0&24.2&1.237&0.504&74.2&74.2&27.6&1.085&0.606&75.1&75.1&28.9&1.029&0.609&74.2&74.3&32.2&1.039&0.625&75.4&75.4&31.9&0.999&0.644\\
%\Xhline{0.5\arrayrulewidth}
%$\Delta^{SOTA}$	& $\uparrow $  & \\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on CMU-MOSI dataset. Epochs determined by validation set, batchsize 128, Adam optimizer, learning rate 0.001.}
\label{mosi2}
\end{table}

==> tables2/sst0.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{SST} 5 Class Sentiment Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & DAN Small & DAN Large & LSTM Small & LSTM Large  \\ 
\Xhline{0.5\arrayrulewidth}
%no shuffle &42.94&41.72&\textbf{41.49}&\textbf{42.53}&\textbf{43.17}\\
shuffle
&43.03&\textbf{41.77}&39.41&41.36&42.26\\
%inc&43.30&41.54&40.23&41.85&42.40\\
dec
&\textbf{43.26}&40.95&40.54&39.86&40.95\\
dec, swr&42.76&41.58&39.14&39.95&40.72\\
dec, swor&42.80&\textbf{41.77}&40.63&40.91&42.76\\
%inc, samp w rep&\textbf{43.58}&41.31&41.27&41.31&\textbf{44.03}\\
%inc, samp wo rep&42.99&\textbf{41.90}&39.37&41.90&42.17\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on SST dataset. Epochs determined by validation set, batchsize 256, Adam optimizer, learning rate 0.001.}
\label{sst0}
\end{table}

==> tables2/sst2.tex <==
\begin{table}[ht!]
\fontsize{7}{10}\selectfont
\centering
\setlength\tabcolsep{9.35pt}
\begin{tabular}{l : c c c c c}
\Xhline{3\arrayrulewidth}
Task & \multicolumn{5}{c}{\textbf{SST} 5 Class Sentiment Classification Accuracy (\%)} \\
%\cmidrule(lr{.5em}){2-3} \cmidrule(lr{.5em}){4-4} \cmidrule(lr{.5em}){5-6}
Method       & LR & DAN Small & DAN Large & LSTM Small & LSTM Large  \\ 
\Xhline{0.5\arrayrulewidth}
no shuffle&38.82&40.41&36.29&37.38&35.57\\
shuffle&38.55&42.90&42.67&43.71&\textbf{44.80}\\
%&38.82&42.99&42.35&45.66&44.21\\
dec&\textbf{39.05}&42.35&\textbf{42.85}&\textbf{45.84}&43.85\\
dec, samp w rep&39.05&42.67&41.81&44.80&44.66\\
dec, samp wo rep&38.82&\textbf{43.35}&41.72&45.02&\textbf{44.80}\\
%inc, samp w rep&38.55&\textbf{43.12}&42.35&43.94&\textbf{45.38}\\
%inc, samp wo rep&38.33&42.49&41.49&45.75&40.23\\
\Xhline{3\arrayrulewidth}
\end{tabular}
\caption{Results on SST dataset. Epochs determined by validation set, batchsize 256, SGD optimizer, learning rate 0.01.}
\label{sst2}
\end{table}
